Solving Multi-Structured Problems by Introducing Linkage Kernels into GOMEA

Model-Based Evolutionary Algorithms (MBEAs) can be highly scalable by virtue of linkage (or variable interaction) learning. This requires, however, that the linkage model can capture the exploitable structure of a problem. Usually, a single type of linkage structure is attempted to be captured using models such as a linkage tree. However, in practice, problems may exhibit multiple linkage structures. This is for instance the case in multi-objective optimization when the objectives have different linkage structures. This cannot be modelled sufficiently well when using linkage models that aim at capturing a single type of linkage structure, deteriorating the advantages brought by MBEAs. Therefore, here, we introduce linkage kernels, whereby a linkage structure is learned for each solution over its local neighborhood. We implement linkage kernels into the MBEA known as GOMEA that was previously found to be highly scalable when solving various problems. We further introduce a novel benchmark function called Best-of-Traps (BoT) that has an adjustable degree of different linkage structures. On both BoT and a worst-case scenario-based variant of the well-known MaxCut problem, we experimentally find a vast performance improvement of linkage-kernel GOMEA over GOMEA with a single linkage tree as well as the MBEA known as DSMGA-II.

==> tables/2021-12-23-paper_bot_vs_maxcut_oac_evaluations_significant.tex <==
\begin{tabular}{llrrrrrr}
\toprule
{} & {approach_y} & {Objective / Domination} & {Objective / Scalarized} & {Asymmetric Kernel / Domination} & {Asymmetric Kernel / Scalarized} & {Symmetric Kernel / Domination} & {Symmetric Kernel / Scalarized} \\
{fns} & {approach_x} & {} & {} & {} & {} & {} & {} \\
\midrule
\multirow[c]{6}{*}{1} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.121 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.856 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.541 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.022 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.879 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.993 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.938 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.144 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.007 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.104 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.459 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.062 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.896 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.978 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\multirow[c]{6}{*}{2} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.633 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.057 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.988 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.559 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Objective / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.367 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.076 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.873 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.395 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.943 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.924 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.970 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.012 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.127 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.441 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.605 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.030 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\multirow[c]{6}{*}{4} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.998 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.622 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.997 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.339 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.378 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.997 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.003 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.661 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.003 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\multirow[c]{6}{*}{8} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.639 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.987 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.361 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.995 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.435 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.013 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.005 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.565 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\bottomrule
\end{tabular}


==> tables/2021-12-23-paper_bot_vs_maxcut_oac_time_significant.tex <==
\begin{tabular}{llrrrrrr}
\toprule
{} & {approach_y} & {Objective / Domination} & {Objective / Scalarized} & {Asymmetric Kernel / Domination} & {Asymmetric Kernel / Scalarized} & {Symmetric Kernel / Domination} & {Symmetric Kernel / Scalarized} \\
{fns} & {approach_x} & {} & {} & {} & {} & {} & {} \\
\midrule
\multirow[c]{6}{*}{1} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.015 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.121 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.097 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.853 \\
 & Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.985 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.941 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.856 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.879 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.059 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.350 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.903 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.144 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.650 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.147 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\multirow[c]{6}{*}{2} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.792 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.049 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.009 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.926 \\
 & Objective / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.208 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.005 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.011 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.008 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.302 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.995 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.940 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.951 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.989 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.024 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.991 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.992 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.060 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.976 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.074 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.698 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\multirow[c]{6}{*}{4} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.147 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.747 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.524 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.004 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.987 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.853 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.998 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.476 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.253 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.996 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.013 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\multirow[c]{6}{*}{8} & Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.996 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.992 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.004 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.204 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.756 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.008 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.796 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.984 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.752 \\
 & Symmetric Kernel / Domination & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.244 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.016 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
 & Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.248 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\bottomrule
\end{tabular}


==> tables/2021-12-23-paper_maxcut_vs_maxcut_oac_evaluations_significant.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{approach_y} & {Objective / Domination} & {Objective / Scalarized} & {Asymmetric Kernel / Domination} & {Asymmetric Kernel / Scalarized} & {Symmetric Kernel / Domination} & {Symmetric Kernel / Scalarized} \\
{approach_x} & {} & {} & {} & {} & {} & {} \\
\midrule
Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.006 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.951 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.002 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.981 \\
Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.994 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.998 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.049 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.019 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\bottomrule
\end{tabular}


==> tables/2021-12-23-paper_maxcut_vs_maxcut_oac_time_significant.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{approach_y} & {Objective / Domination} & {Objective / Scalarized} & {Asymmetric Kernel / Domination} & {Asymmetric Kernel / Scalarized} & {Symmetric Kernel / Domination} & {Symmetric Kernel / Scalarized} \\
{approach_x} & {} & {} & {} & {} & {} & {} \\
\midrule
Objective / Domination & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.021 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.887 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Objective / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.001 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.121 \\
Asymmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.979 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Asymmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.999 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Symmetric Kernel / Domination & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.113 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 1.000 \\
Symmetric Kernel / Scalarized & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{808080}} \color[HTML]{FFFFFF} 0.879 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{FFFFFF}} \color[HTML]{000000} 0.000 & {\cellcolor[HTML]{D3D3D3}} \color[HTML]{000000} - \\
\bottomrule
\end{tabular}

